CMT: Mid-Training for Efficient Learning of Consistency, Mean Flow, and Flow Map Models

Flow map models such as Consistency Models (CM) and Mean Flow (MF) enable few-step generation by learning the long jump of the ODE solution of diffusion models, yet training remains unstable, sensitive to hyperparameters, and costly. Initializing from a pre-trained diffusion model helps, but still requires converting infinitesimal steps into a long-jump map, leaving instability unresolved. We introduce mid-training, the first concept and practical method that inserts a lightweight intermediate stage between the (diffusion) pre-training and the final flow map training (i.e., post-training) for vision generation. Concretely, Consistency Mid-Training (CMT) is a compact and principled stage that trains a model to map points along a solver trajectory from a pre-trained model, starting from a prior sample, directly to the solver-generated clean sample. It yields a trajectory-consistent and stable initialization. This initializer outperforms random and diffusion-based baselines and enables fast, robust convergence without heuristics. Initializing post-training with CMT weights further simplifies flow map learning. Empirically, CMT achieves state of the art two step FIDs: 1.97 on CIFAR-10, 1.32 on ImageNet 64x64, and 1.84 on ImageNet 512x512, while using up to 98% less training data and GPU time, compared to CMs. On ImageNet 256x256, CMT reaches 1-step FID 3.34 while cutting total training time by about 50% compared to MF from scratch (FID 3.43). This establishes CMT as a principled, efficient, and general framework for training flow map models.

==> cmt_benefits.tex <==
\subsection{Summary: Practical Advantages of Mid-Training with \methods} 

% \begin{figure}[th!]
%     \centering % Center the entire figure content

%     % --- First Subfigure ---
%     \begin{minipage}{0.31\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{example-image-a}
%         \subcaption{First subfigure}
%         \label{fig:sub1}
%     \end{minipage}\hfill % \hfill creates horizontal space between the minipages
%     % --- NO BLANK LINE HERE ---
%     % --- Second Subfigure ---
%     \begin{minipage}{0.31\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{example-image-b}
%         \subcaption{Second subfigure}
%         \label{fig:sub2}
%     \end{minipage}\hfill % --- NO BLANK LINE HERE ---
%     % --- Third Subfigure ---
%     \begin{minipage}{0.31\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{example-image-c}
%         \subcaption{Third subfigure}
%         \label{fig:sub3}
%     \end{minipage}

%     \caption{This is the main caption for all three subfigures.}
%     \label{fig:main}
% \end{figure}

% Unlike conventional flow map models such as CMs and MF, the mid-training loss of \methods requires no stop-gradients, specialized time-sampling, or handcrafted loss weights $w(t)$. 
% %Regarding the ODE solver, we use a high-order DPM-Solver++ \cite{lu2022dpm++} with 16 steps in all EDM-based CMs, and a second-order Heun solver with 16 steps in flow-based models, which efficiently generates high-fidelity labels and accurate trajectories within limited steps. 
% The identical ODE solver works well for a broad class of flow map learning models thanks to their strong theoretical guarantee in the ODE literature \cite{lu2022dpm,lu2022dpm++}.
% Empirically, we find that \methods trains quickly and stably, while also providing strong initialization that significantly improves the final stage of flow map learning, leading to superior performance.

% Many pre-trained diffusion models are available, including research-purpose models \cite{karras2022edm, karras2024edm2, ma2024sit, peebles2023dit} and industrial-level models like Stable Diffusion (SD) \cite{rombach2022high} and FLUX \cite{flux2024,labs2025flux1kontextflowmatching}. Recycling these models with a simple CMT step can achieve SOTA performance. This approach avoids the computational demands of training everything from scratch, like Mean Flow \cite{geng2025mean} and iCT \cite{song2023ict}. \jcc{because we never tried our method on,  mentioning all the off-the-shelf diffusion model may be tricky, especially the T2I models. }

% \methods can also be implemented easily for various flow map learning frameworks and pre-trained diffusion models. The pseudocode is provided in Algorithm 1.
% %
% Given an arbitrary pre-trained diffusion model equipped with an ODE solver, we generate the numerical ODE trajectory, which serves as the label for \methods supervision.
% %
% \methods is thus more general than other flow-map learning algorithms focusing on one diffusion process only, either EDM or Flow. 

% Our methods can be divided into several stages. The entire training pipeline is summarized in Algorithm 2.



% \textbf{Low Cost of \method.} The main computational bottleneck of \methods is the non-parallelizable multistep ODE solver generating the reference ODE trajectory. However, thanks to SOTA few-step ODE solvers like DPM-Solver~\citep{lu2022dpm,lu2022dpm++} and Heun solver~\citep{karras2022edm}, we just use 16 steps to efficiently generate high-fidelity regression targets and accurate trajectories within limited steps.
% %
% This makes \method's speed similar to consistency distillation (CD) and is just 15\%$\sim$25\% slower than consistency training (CT), as observed in our comparison for \method, CT, and CD, using the Easy CT (ECT) and Easy CD (ECD)~\citep{geng2024ect} as examples due to their relatively more straightforward configurations. More empirical details are provided in Appendix \ref{appendix:speed}.
% %
% Theoretically, 
% \begin{itemize}
% \item \textbf{CT} requires computing $\rvf_{\btheta}(\rvx_t, t)$ (backpropagated) and $\rvf_{\btheta^-}(\rvx_r, r)$ (detached from GPU), where $r = t - \Delta t$.
% \textbf{CD} requires what CT needs, plus several additional inferences from the detached one-step solver to obtain $\rvx_r$.
% \item \textbf{\method} fits $\rvf_\btheta(\rvx_t, t)$ (backpropagated) to the solver-generated target $\hat{\rvx}_0$. 
% Each teacher model evaluation in the detached ODE-Solver contributes to one training sample on the ODE trajectory. 
% Hence, \methods requires two model evaluations for one data: one backpropagated and another detached from the ODE-Solver. This theoretical cost is identical to CT.
% However, ODE-Solver cannot be parallelized, making it slightly slower than CT.
% \end{itemize}
% Nevertheless, if we pre-generate the DPM-Solver trajectory, then \methods only requires one backpropagated model evaluation, which is the fastest among all, adopted by previous diffusion distillation work \cite{zheng2023dfno}.
% %
% But pre-generation requires additional preparation and storage. 
% %
% Thus, all our experiments run the ODE-Solver during training and do not pre-generate.

% Furthermore, the number of function evaluations (NFEs) or steps in the ODE-Solver is also crucial to \method's speed, as a lack of parallelization in the ODE-Solver is the main speed bottleneck.
% %
% Larger NFE leads to a greater lack of parallelization, resulting in \methods being slower.
% %
% Hence, we choose NFE = 16 in all experiments, which is sufficient for pretraining and is only slightly slower than CT.
% %
% DPM-Solver++~\citep{lu2022dpm++} (for CM) or Heun solver (for MeanFlow)~\citep{karras2022edm} is chosen thanks to its stability under the low NFE regime.

% Choosing a small NFE will still be sufficient for \method, whose error is from (1) distillation fitting error due to the non-zero loss value; and (2) error from the small NFE and the teacher diffusion model.
% In practice, we found that (1) is the main obstacle.
% %
% DPM-Solver with 16 NFEs performs just slightly worse than the best FID under a large NFE.
% The FID gap is usually 0.2.
% Hence, \methods with the 16 NFEs DPM-Solver is fast and good.

\textbf{Generality and Cost Efficiency for Flow Map Learning.}
\methods is a general approach to flow map learning that is both computationally and economically efficient. 
Training flow map models entirely from scratch is prohibitively expensive, as demonstrated by iCT \cite{song2023ict}, ECM \cite{geng2024ect}, and Mean Flow~\citep{geng2025mean}. 
In contrast, a wide range of pre-trained diffusion models are already available~\citep{karras2022edm, karras2024edm2, ma2024sit, peebles2023dit}.%, from recent architectures~\citep{karras2022edm, karras2024edm2, ma2024sit, peebles2023dit} to widely adopted large-scale checkpoints such as Stable Diffusion~\citep{rombach2022high} and FLUX~\citep{flux2024,labs2025flux1kontextflowmatching}. 
By generating numerical ODE trajectories from such pre-trained models with a high-order solver like DPM-Solver++~\citep{lu2022dpm++}, \methods recycle existing models through a simple \methods step. 
This avoids costly retraining and yields competitive or even superior results with only a few generation steps, making the approach especially appealing under limited compute and data budgets.



\textbf{Simplicity and Stability.}
In contrast to conventional flow-map models like CMs and MF, the mid-training loss of \methods uses an explicit regression target, avoiding the need for stop-gradients, specialized time sampling, or handcrafted weights $w(t)$. Thus, \method's training is stable.
The pseudocode is provided in \Cref{app:algorithm}. 
Empirically, we observe that \methods trains quickly and stably, while also providing a strong initialization that accelerates and improves the final stage of flow map learning. 
\jcc{See XXX for results.} \zh{This is reflected in all experiments where \methods is better than pure flow map learning and \methods reaches SOTA. More specifically, in CM settings, including CIFAR10, ImageNet 64$\times$64 and 512$\times$512, AFHQv2 and FFHQ, we use ECM \cite{geng2024ect} as the post-training flow map learning method. \methods with ECM significantly outperforms pure ECM. Further, \methods with MF \cite{geng2025mean} also outperforms pure MF on ImageNet 256$\times$256.}

\textbf{Low Cost of \method.}
Although \methods requires a sequential multistep ODE solver to generate reference trajectories, modern few-step solvers such as DPM-Solver~\citep{lu2022dpm,lu2022dpm++} and the Heun solver~\citep{karras2022edm} allow us to produce high-fidelity regression targets with only about 16 steps. Moreover, the multistep formulation enables us to recycle previously computed states $\hat\rvx_{t_k}$ for constructing later states $\hat\rvx_{t_i}$, which further reduces overhead. As a result, \methods can achieve training efficiency on par with consistency distillation (CD), requiring additional teacher inference cost, and continuous consistency training (CT), requiring JVP computation. 
And \methods is observed to be only 15\%--25\% slower than discrete CT under the formulation of \citep{geng2024ect} per iteration; while \methods is significantly more stable 
\jcc{can we say CMT needs fewer iterations to converge, hence, the real runtime is much fewer??}. \zh{Thus, \methods needs fewer iterations to converge by reducing training data cost. In turn, \methods can save GPU run time since \methods per iteration speed is similar to other baselines. This advantage is especially obvious on ImageNet 64$\times$64 and 512$\times$512, where we achieve SOTA performance while reducing 75$\%$ to 98$\%$ training data cost and GPU time.}


We also measure compute on a per-pair basis, where a ``pair'' is one input–target example used in training. In \methods, a single teacher-generated trajectory provides many pairs by matching intermediate states to the clean target, while in CD and CT each pair is generated independently from a sampled time. Under this view, \methods requires about one teacher call plus one student forward and one backpropagation per pair, CD requires one teacher calls plus the same student cost, and CT requires no teacher calls but two student forwards and one backpropagation. Thus, \methods is roughly as costly as CD and only slightly slower than CT, consistent with our empirical findings. More details are provided in Appendix~\ref{appendix:speed}. 



% \textbf{\methods{} Adapts to Flexible Teacher–Student Architectures. }
% Furthermore, \methods is flexible in accommodating teacher and student models with different network architectures, a setting where many existing approaches fail. For example, the diffusion initialization strategy, which relies on initializing the flow map model from a pre-trained diffusion model, breaks down when teacher and student architectures differ and is particularly unsuitable for distilling a large model into a smaller one. In contrast, \methods allows us to randomly initialize a compact student and leverage the ODE trajectory generated by a larger diffusion or flow model to guide its mid-training. We validate this property in practice by successfully transferring an extra-large MeanFlow-XL/2~\cite{geng2025mean} into a Base-size MeanFlow-B/2.
% \jcc{See XXX for results.} \zh{Added to MF experiment.}




% Furthermore, \methods is also flexible with teacher and student models with distinct neural network structures, while other methods cannot. For instance, the diffusion-initialization trick, i.e., initializing the flow map model with a pre-trained diffusion model, cannot adapt to teacher and student models with different configurations, especially when we want to distill a large model to a small one in practice. In contrast, we can randomly initialize a small model and then use the ODE trajectory of another large diffusion/flow model for \methods mid-training the small one. We testify this in experiments via transferring an extra-large MeanFlow-XL/2 \cite{geng2025mean} to a Base size MeanFlow-B/2.


% \textbf{\methods as a Data-Free Distillation Method (Appendix). }
% \methods itself can be viewed as a standalone data-free distillation method without engineering heuristics, especially showing competitive performances in high-dimensional scenarios where other flow map models become increasingly unstable. A byproduct is that it is data-free in the mid-training stage; thus, it potentially support the data-free training for the flow map model


==> experiments.tex <==
\section{Experimental Results}
\subsection{Mid-Training with \methods Improves Flow Map Post-Training}
\begin{comment}
\begin{table}[t]
\centering
\caption{\small{Sample quality on unconditional CIFAR10 32$\times$32 and class-conditional ImageNet 64$\times$64.}}
\label{tab:cifar_imgnet64}
\begin{minipage}{0.48\textwidth}
\fontsize{7.52pt}{8.52pt}\selectfont
%\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcc}
\multicolumn{3}{l}{\textbf{Unconditional CIFAR10 32$\times$32}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion \& Fast Samplers}} \\
\midrule
%Score SDE (deep)~\citep{song2020score} & 2000 & 2.20 \\
EDM~\citep{karras2022edm} & 35 & 2.01 \\
% Flow Matching~\citep{lipman2022flowmatching} & 142 & 6.35 \\
%OT-CFM~\citep{tong2023improving} & 1000 & 3.57 \\
% DPM-Solver~\citep{lu2022dpm} & 10 & 4.70 \\
% DPM-Solver++~\citep{lu2022dpm++} & 10 & 2.91 \\
DPM-v3~\citep{zheng2023dpmv3} & 10 & 2.51 \\
\midrule
\multicolumn{3}{l}{\textbf{Joint Training}} \\
\midrule
% Diffusion GAN~\citep{xiao2021diffusion-GAN} & 4 & 3.75 \\
% Diffusion StyleGAN~\citep{wang2022diffusion-stylegan} & 1 & 3.19 \\
CTM~\citep{kim2023ctm} & 1 & \textbf{1.87} \\
% Diff-Instruct~\citep{luo2024diff-instruct} & 1 & 4.53 \\
DMD~\citep{yin2024dmd} & 1 & 3.77 \\
SiD~\citep{zhou2024SiD} & 1 & 1.92 \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion Distillation}} \\
\midrule
DFNO~\citep{zheng2023dfno} & 1 & 3.78 \\
2-Rectified Flow~\citep{rectified_flow} & 1 & 4.85 \\
TRACT~\citep{berthelot2023tract} & 1 & 3.78 \\
& 2 & 3.32 \\
PD~\citep{salimans2022progressive} & 1 & 8.34 \\
& 2 &5.58 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Flow Maps via Distillation}} \\
% \midrule
CD~\citep{song2023cm} & 1 & 3.55 \\
 & 2 & 2.93 \\
sCD~\citep{lu2025sCM} & 1 & 3.66 \\
& 2 & 2.52 \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Maps from Scratch}} \\
\midrule
iCT~\citep{song2023ict} & 1 & 2.83 \\
& 2 & 2.46 \\
iCT-deep~\citep{song2023ict} & 1 & 2.51 \\
& 2 & 2.24 \\
ECT~\citep{geng2024ect} & 1 & 3.60 \\
& 2 & 2.11 \\
{sCT~\citep{lu2025sCM}} & 1 & 2.85 \\
& 2 & 2.06 \\
Stable CT~\citep{wang2024stable} & 1 & 2.92 \\
& 2 & 2.02 \\
VCT~\citep{silvestri2025vct} & 1 & 3.26 \\
& 2 & 2.02 \\
{TCM~\citep{lee2024TCM}} & 1 & \textbf{2.46} \\
& 2 & 2.05 \\
IMM~\citep{zhou2025inductive} & 1 & 3.20 \\
 & 2 & 1.98 \\
 MF~\citep{geng2024ect} & 1 & 2.92 \\
\midrule
\multicolumn{3}{l}
{\textbf{\fmethod\ (\method)}} \\
\midrule
% \rowcolor{tgray}
% \method\ (Ours) & 1 & 5.71 \\
% \rowcolor{tgray}
%  & 2 & 4.65 \\
 \rowcolor{torange}
 \method\ (w/ ECT) (Ours) & 1 & 2.74 \\
  \rowcolor{torange}
 & 2 & \textbf{1.97} \\
\bottomrule
\end{tabular} %
}
\end{minipage}
\begin{minipage}{0.48\textwidth}
\fontsize{7.52pt}{8.52pt}\selectfont
%\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcc}
\multicolumn{3}{l}{\textbf{Class-Conditional ImageNet 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion \& Fast Samplers}} \\
\midrule
% ADM~\citep{diffusion_beat_gan} & 250 & 2.07 \\
RIN~\citep{jabri2022rin} & 1000 & 1.23 \\
% DPM-Solver~\citep{lu2022dpm} & 20 & 3.42 \\
%EDM (Heun)~\citep{karras2022edm} & 79 & 2.44 \\
EDM2~\citep{karras2024edm2} & 63 & 1.33 \\
\midrule
\multicolumn{3}{l}{\textbf{Joint Training}} \\
\midrule
% StyleGAN-XL~\citep{sauer2022stylegan-xl} & 1 & 1.52 \\
% Diff-Instruct~\citep{luo2024diff-instruct} & 1 & 5.57 \\
EMD~\citep{xie2024EMD} & 1 & 2.20 \\
%DMD~\citep{yin2024dmd} & 1 & 2.62 \\
DMD2~\citep{yin2024dmd2} & 1 & \textbf{1.28} \\
SiD~\citep{zhou2024SiD} & 1 & 1.52 \\
CTM~\citep{kim2023ctm} & 1 & 1.92 \\
& 2 & 1.73 \\
% Moment Matching~\citep{salimans2024multistepmoment} & 1 & 3.00 \\
% & 2 & 3.86 \\
% AYF + adv. loss~\citep{sabour2025align} & 1 & 1.32 \\
% & 2 & 1.17 \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion Distillation}} \\
\midrule
DFNO~\citep{zheng2023dfno} & 1 & 7.83 \\
% PID (LPIPS)~\citep{tee2024PID} & 1 & 9.49 \\
TRACT~\citep{berthelot2023tract} & 1 & 7.43 \\
& 2 & 4.97 \\
PD~\citep{salimans2022progressive} & 1 & 10.70 \\
%\quad\quad (reimpl. from \citet{heek2024multistepcm}) 
& 2 & 4.70 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Flow Maps via Distillation}} \\
% \midrule
CD~\citep{song2023cm} & 1 & 6.20 \\
& 2 & 4.70 \\
MultiStep-CD~\citep{heek2024multistepcm} & 1 & 3.20 \\
& 2 & 1.90 \\
sCD~\citep{lu2025sCM} & 1 & 2.44 \\
& 2 & 1.66 \\
% AYF~\citep{sabour2025align} & 1 & 2.98 \\
% & 2 & 1.25 \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Maps from Scratch}} \\
\midrule
% CTM~\citep{kim2023ctm} & 1 & 1.92 \\
% & 2 & 1.73 \\
iCT~\citep{song2023ict} & 1 & 4.02 \\
& 2 & 3.20 \\
iCT-deep~\citep{song2023ict} & 1 & 3.25 \\
& 2 & 2.77 \\
ECT~\citep{geng2024ect} & 1 & 2.49 \\
& 2 & 1.67 \\
sCT~\citep{lu2025sCM} & 1 & 2.04 \\
& 2 & 1.48 \\
Stable CT~\citep{wang2024stable} & 1 & 2.42 \\
& 2 & 1.55 \\
VCT~\citep{silvestri2025vct} & 1 & 4.93 \\
& 2 & 3.07 \\
{TCM~\citep{lee2024TCM}} & 1 & 2.20 \\
& 2 & 1.62 \\
\midrule
\multicolumn{3}{l}
{\textbf{\fmethod\ (\method)}} \\
\midrule
% \rowcolor{tgray}
% \method\ (Ours) & 1 & 6.00 \\ 
% \rowcolor{tgray}
%  & 2 & 3.87 \\ 
\rowcolor{torange}
 \method\ (w/ ECT) (Ours) & 1 & \textbf{2.02} \\ \rowcolor{torange}
 & 2 & \textbf{1.48} \\
 % \rowcolor{torange}
 % \method\ (w/ ECD) (Ours) & 1 & \textbf{1.93} \\ \rowcolor{torange}
 % & 2 & \textbf{1.42} \\
\bottomrule
\end{tabular} %
}
\end{minipage}
\vspace{-.2in}
\end{table}
\end{comment}

\begin{table}[t]
\centering
\caption{\small{Sample quality on unconditional CIFAR10 32$\times$32 and class-conditional ImageNet 64$\times$64.}}
\label{tab:cifar_imgnet64}
\begin{minipage}{0.495\textwidth}
\fontsize{8.5pt}{9.5pt}\selectfont
{%
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip -5pt}c@{\hskip 5pt}c}
\multicolumn{3}{l}{\textbf{Unconditional CIFAR10 32$\times$32}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion \& Fast Samplers}} \\
\midrule
%Score SDE (deep)~\citep{song2020score} & 2000 & 2.20 \\
EDM~\citep{karras2022edm} & 35 & 2.01 \\
% Flow Matching~\citep{lipman2022flowmatching} & 142 & 6.35 \\
%OT-CFM~\citep{tong2023improving} & 1000 & 3.57 \\
% DPM-Solver~\citep{lu2022dpm} & 10 & 4.70 \\
% DPM-Solver++~\citep{lu2022dpm++} & 10 & 2.91 \\
DPM-v3~\citep{zheng2023dpmv3} & 10 & 2.51 \\
\midrule
\multicolumn{3}{l}{\textbf{Joint Training}} \\
\midrule
% Diffusion GAN~\citep{xiao2021diffusion-GAN} & 4 & 3.75 \\
% Diffusion StyleGAN~\citep{wang2022diffusion-stylegan} & 1 & 3.19 \\
CTM~\citep{kim2023ctm} & 1 & \textbf{1.87} \\
% Diff-Instruct~\citep{luo2024diff-instruct} & 1 & 4.53 \\
DMD~\citep{yin2024dmd} & 1 & 3.77 \\
SiD~\citep{zhou2024SiD} & 1 & 1.92 \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion Distillation}} \\
\midrule
DFNO~\citep{zheng2023dfno} & 1 & 3.78 \\
2-Rectified Flow~\citep{rectified_flow} & 1 & 4.85 \\
TRACT~\citep{berthelot2023tract} & 1 / 2 & 3.78 / 3.32 \\
PD~\citep{salimans2022progressive} & 1 / 2 & 8.34 / 5.58 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Flow Maps via Distillation}} \\
% \midrule
CD~\citep{song2023cm} & 1 / 2 & 3.55 / 2.93 \\
sCD~\citep{lu2025sCM} & 1 / 2 & 3.66 / 2.52 \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Maps from Scratch}} \\
\midrule
iCT~\citep{song2023ict} & 1 / 2 & 2.83 / 2.46 \\
iCT-deep~\citep{song2023ict} & 1 / 2 & 2.51 / 2.24 \\
ECT~\citep{geng2024ect} & 1 / 2 & 3.60 / 2.11 \\
{sCT~\citep{lu2025sCM}} & 1 / 2 & 2.85 / 2.06 \\
Stable CT~\citep{wang2024stable} & 1 / 2 & 2.92 / 2.02 \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 3.26 / 2.02 \\
{TCM~\citep{lee2024TCM}} & 1 / 2 & \textbf{2.46} / 2.05 \\
IMM~\citep{zhou2025inductive} & 1 / 2 & 3.20 / 1.98 \\
 MF~\citep{geng2024ect} & 1 & 2.92 \\
% \midrule
% \multicolumn{3}{l}
% {\textbf{\fmethod\ (\method)}} \\
% \midrule
% \rowcolor{tgray}
% \method\ (Ours) & 1 & 5.71 \\
% \rowcolor{tgray}
%  & 2 & 4.65 \\
 \rowcolor{torange}
 \method\ (w/ ECT) (Ours) & 1 / 2 & 2.74 / \textbf{1.97} \\
\bottomrule
\end{tabular} %
}
\end{minipage}
\begin{minipage}{0.495\textwidth}
\fontsize{8.5pt}{9.5pt}\selectfont
{%
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip -5pt}c@{\hskip 5pt}c}
\multicolumn{3}{l}{\textbf{Class-Conditional ImageNet 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion \& Fast Samplers}} \\
\midrule
% ADM~\citep{diffusion_beat_gan} & 250 & 2.07 \\
RIN~\citep{jabri2022rin} & 1000 & 1.23 \\
% DPM-Solver~\citep{lu2022dpm} & 20 & 3.42 \\
%EDM (Heun)~\citep{karras2022edm} & 79 & 2.44 \\
EDM2~\citep{karras2024edm2} & 63 & 1.33 \\
\midrule
\multicolumn{3}{l}{\textbf{Joint Training}} \\
\midrule
% StyleGAN-XL~\citep{sauer2022stylegan-xl} & 1 & 1.52 \\
% Diff-Instruct~\citep{luo2024diff-instruct} & 1 & 5.57 \\
EMD~\citep{xie2024EMD} & 1 & 2.20 \\
%DMD~\citep{yin2024dmd} & 1 & 2.62 \\
DMD2~\citep{yin2024dmd2} & 1 & \textbf{1.28} \\
SiD~\citep{zhou2024SiD} & 1 & 1.52 \\
CTM~\citep{kim2023ctm} & 1 / 2 & 1.92 / 1.73 \\
% Moment Matching~\citep{salimans2024multistepmoment} & 1 & 3.00 \\
% & 2 & 3.86 \\
% AYF + adv. loss~\citep{sabour2025align} & 1 & 1.32 \\
% & 2 & 1.17 \\
\midrule
\multicolumn{3}{l}{\textbf{Diffusion Distillation}} \\
\midrule
DFNO~\citep{zheng2023dfno} & 1 & 7.83 \\
% PID (LPIPS)~\citep{tee2024PID} & 1 & 9.49 \\
TRACT~\citep{berthelot2023tract} & 1 / 2 & 7.43 / 4.97 \\
PD~\citep{salimans2022progressive} & 1 / 2 & 10.70 / 4.70 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Flow Maps via Distillation}} \\
% \midrule
CD~\citep{song2023cm} & 1 / 2 & 6.20 / 4.70 \\
MultiStep-CD~\citep{heek2024multistepcm} & 1 / 2 & 3.20 / 1.90 \\
sCD~\citep{lu2025sCM} & 1 / 2 & 2.44 / 1.66 \\
% AYF~\citep{sabour2025align} & 1 & 2.98 \\
% & 2 & 1.25 \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Maps from Scratch}} \\
\midrule
% CTM~\citep{kim2023ctm} & 1 & 1.92 \\
% & 2 & 1.73 \\
iCT~\citep{song2023ict} & 1 / 2 & 4.02 / 3.20 \\
iCT-deep~\citep{song2023ict} & 1 / 2 & 3.25 / 2.77 \\
ECT~\citep{geng2024ect} & 1 / 2 & 2.49 / 1.67 \\
sCT~\citep{lu2025sCM} & 1 / 2 & 2.04 / 1.48 \\
Stable CT~\citep{wang2024stable} & 1 / 2 & 2.42 / 1.55 \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 4.93 / 3.07 \\
{TCM~\citep{lee2024TCM}} & 1 / 2 & 2.20 / 1.62 \\
% \midrule
% \multicolumn{3}{l}
% {\textbf{\fmethod\ (\method)}} \\
% \midrule
% \rowcolor{tgray}
% \method\ (Ours) & 1 & 6.00 \\ 
% \rowcolor{tgray}
%  & 2 & 3.87 \\ 
\rowcolor{torange}
 \method\ (w/ ECT) (Ours) & 1 / 2 & \textbf{2.02} / \textbf{1.48} \\
 % \rowcolor{torange}
 % \method\ (w/ ECD) (Ours) & 1 & \textbf{1.93} \\ \rowcolor{torange}
 % & 2 & \textbf{1.42} \\
\bottomrule
\end{tabular} %
}
\end{minipage}
\vspace{-.2in}
\end{table}

\textbf{Datasets and Setup}. We validate our method on various datasets: CIFAR10 (32$\times$32)~\citep{krizhevsky2009cifar}, AFHQv2 (64$\times$64) and FFHQ (64$\times$64)~\citep{karras2022edm}, ImageNet~\citep{deng2009imagenet} with three resolutions (64$\times$64, 256$\times$256, and 512$\times$512).
%
We follow EDM~\citep{karras2022edm}, ECT~\citep{geng2024ect}, and VCT~\citep{silvestri2025vct} on low-resolution unconditional datasets, namely CIFAR10, AFHQv2, and FFHQ.
%
Meanwhile, the EDM2~\citep{karras2024edm2} setting is adopted for ImageNet 64$\times$64 and 512$\times$512, where we use the Stable Diffusion (SD) autoencoder to learn the 512$\times$512 generation in a latent space.
%
We follow the Mean Flow~\citep{geng2025mean} and SiT~\citep{ma2024sit} settings for ImageNet 256$\times$256, which also uses SD for latent generation.
%

\method\ mid-training's teacher diffusion model is EDM with DPM-Solver++ on CIFAR10, AFHQv2, and FFHQ. 
Its teacher becomes EDM2 with DPM-Solver++ on ImageNet 64$\times$64 and 512$\times$512. 
Its teacher is SiT with a second-order Heun solver on ImageNet 256$\times$256.

After \method's mid-training, we use ECT for post-training in CIFAR10, AFHQv2, FFHQ, and ImageNet 64$\times$64 since they follow EDM and ECT is designed for EDM-type CM.
%
We use Mean Flow for ImageNet 256$\times$256 post-training as it is the latest SOTA flow map in this case.
%
Lastly, we use ECD post-training for ImageNet 512$\times$512 as CD is proven to be more stable and effective in very high-dimensional image generation than CT~\citep{lu2025sCM}.



We benchmark models using Fréchet Inception Distance (FID)~\citep{heusel2017fid}. The cost of training data, measured in millions of images (Mimgs), is used to test data efficiency, and training GPU time is used for benchmarking convergence time.
%
More details are provided in the Appendix \ref{appendix:exp_detail}, but we keep the hyperparameters as simple as possible, e.g., deleting the sophisticated $\Delta t$ annealing, loss weighting, time sampling trick, power function EMA, nonlinear learning rate scheduler, etc.
%
We use learned perceptual loss for CMT's mid-training throughout all experiments to align the model prediction with the high-fidelity fixed label produced by the teacher. Specifically, we use vanilla LPIPS~\citep{zhang2018lpips} in pixel space and ELatentLPIPS~\citep{kang2024distilling} in latent space.

\textbf{CIFAR10 and ImageNet 64$\times$64}: Table \ref{tab:cifar_imgnet64} demonstrates that our method achieves SOTA with 2-step FID=1.97 on CIFAR10, exceeding the teacher diffusion EDM's 2.01 with 35 steps and most previous CMs and flow maps. 
%
We also achieve the best FIDs across all CMs and flow map models on ImageNet 64$\times$64, and the 2-step FID=1.48 is satisfactorily chosen over EDM's 1.33 with 63 NFEs.
%
%Comparisons with more baselines are in the Appendix, where our method still outperforms.
These excellent SOTA results are also achieved within a limited budget.
%

For {CIFAR10}, we utilize a total training budget of 51.2 Mimgs, with 38.4 Mimgs allocated for mid-training and 12.8 Mimgs for post-training flow map learning. 
%
On CIFAR10, our approach surpasses both ECT and VCT with the identical 51.2 Mimgs total costs. 
sCT uses more budget, and sCT's 1-step FID under the same 51.2 Mimgs budget is just 3.09, which is worse than our 2.74, validating that we are more data-efficient than sCT.
Stable CT requires a significantly larger budget of 153.6 Mimgs and still cannot outperform us at a much lower 51.2 Mimgs cost.
TCM achieves comparable SOTA results to ours, but with a significantly larger budget of 332.8 Mimgs.
%

For 
{ImageNet 64$\times$64}, \methods result is achieved within a tiny 12.8 Mimgs budget with 6.4 allocated to mid-training and 6.4 for post-training flow map learning, while ECT and Stable CT use 102.4 Mimgs, sCT uses 819.2 Mimgs, and TCM uses 143.36 Mimgs.
%
Compared to the previous SOTA sCT, we save up to $98\%$ of training images costs.
Since \method's per-iteration cost is lower than sCT due to sCT's costly Jacobian vector product, \methods achieve SOTA also with $98\%$ lower GPU time.
% Remark: We successfully reproduce the previous SOTA result within a tiny 12.8 Mimgs cost.
%
% \method\ with even smaller costs for fast validation on ImageNet 64$\times$64 is provided in Appendix \ref{appendix:ImageNet_Small_Cost}.

Therefore, our method is both SOTA and data-efficient, ensuring faster convergence.
%
We also delete the complicated $\Delta t$ annealing in common CM training to keep our framework as simple as possible.
%
Notably, \methods using ECT as post-training flow map learning outperforms ECT significantly under the same or even lower budget, proving the \method\ mid-training's importance.
Additional evidence of mid-training's significance is provided in Appendix \ref{appendix:Importance_of_Midtraining}.


\textbf{AFHQv2 and FFHQ 64$\times$64}: Table \ref{tab:ffhq_afhq} further provides a CM comparison given a training data budget of 51.2 Mimgs. 
%
Since AFHQv2 and FFHQ are also unconditioned like CIFAR10, we directly transfer the tuned hyperparameters from CIFAR10 with minor modifications for all CMs.
%`1
Our \methods achieves the best 1-step and 2-step FIDs. %, and its 2-step FID is satisfactorily close to the teacher EDM. 
%
Furthermore, \methods using ECT as post-training flow map learning again outperforms ECT significantly under the same budget.
%
This further validates \method's hyperparameter robustness and mid-training importance across various datasets.

\begin{table}[t]
\centering
\caption{\small{Comparison between various CMs given the identical 51.2 million training images budget on AFHQv2 64$\times$64 and FFHQ 64$\times$64. Our \methods achieve the best 1-step and 2-step FIDs.}}
\label{tab:ffhq_afhq}
\begin{minipage}{0.495\textwidth}
\fontsize{8.25pt}{9.25pt}\selectfont
{%
\begin{tabular}{lcc}
\multicolumn{2}{l}{\textbf{Unconditional AFHQv2 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
% EDM~\citep{karras2022edm} & 79 & 1.96 \\
iCT~\citep{song2023ict} & 1 / 2 & 5.40 / 2.92  \\
ECT~\citep{geng2024ect} & 1 / 2 & 3.89 / 2.61  \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 3.84 / 2.71 \\
\rowcolor{torange}
\methods (w/ ECT) (Ours) & 1 / 2 & \textbf{3.28} / \textbf{2.34} \\
\bottomrule
\end{tabular} %
}

\end{minipage}
\begin{minipage}{0.495\textwidth}
\fontsize{8.25pt}{9.25pt}\selectfont
{%
\begin{tabular}{lcc}
\multicolumn{2}{l}{\textbf{Unconditional FFHQ 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) \\
\midrule
% EDM~\citep{karras2022edm} & 79 & 2.39 \\
iCT~\citep{song2023ict} & 1 / 2 & 5.80 / 4.02 \\
ECT~\citep{geng2024ect} & 1 / 2 & 5.99 / 4.39 \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 5.47 / 4.16 \\
\rowcolor{torange}
\methods (w/ ECT) (Ours) & 1 / 2 & \textbf{3.89} / \textbf{2.75} \\
\bottomrule
\end{tabular} %
}

\end{minipage}
\begin{comment}
\begin{minipage}{0.477\textwidth}
\fontsize{7.55pt}{8.55pt}\selectfont
{%
%\begin{tabular}{lccc}
\begin{tabular}{l@{\hskip 0pt}c@{\hskip 1pt}c@{\hskip 6pt}c}
\multicolumn{3}{l}{\textbf{Unconditional AFHQv2 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) & \textbf{Budget} \\
\midrule
EDM~\citep{karras2022edm} & 79 & 1.96 & N.A. \\
iCT~\citep{song2023ict} & 1 / 2 & 5.40 / 2.92 & 51.2 \\
ECT~\citep{geng2024ect} & 1 / 2 & 3.89 / 2.61 & 51.2 \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 3.84 / 2.71 & 51.2 \\
% \rowcolor{tgray}
% \method\ (Ours) & 1 / 2 & 5.95 / 4.79 & 38.4 \\
\rowcolor{torange}
\methods (w/ ECT) (Ours) & 1 / 2 & \textbf{3.28} / \textbf{2.34} & 51.2 \\
\bottomrule
\end{tabular} %
}

\end{minipage}
\begin{minipage}{0.477\textwidth}
\fontsize{7.55pt}{8.55pt}\selectfont
{%
%\begin{tabular}{lccc}
\begin{tabular}{l@{\hskip 0pt}c@{\hskip 1pt}c@{\hskip 6pt}c}
\multicolumn{3}{l}{\textbf{Unconditional FFHQ 64$\times$64}} \\
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) & \textbf{Budget} \\
\midrule
EDM~\citep{karras2022edm} & 79 & 2.39 & N.A. \\
iCT~\citep{song2023ict} & 1 / 2 & 5.88 / 4.06 & 51.2 \\
ECT~\citep{geng2024ect} & 1 / 2 & 5.99 / 4.39 & 51.2 \\
VCT~\citep{silvestri2025vct} & 1 / 2 & 5.47 / 4.16 & 51.2 \\
% \rowcolor{tgray}
% \method\ (Ours) & 1 / 2 & 7.92 / 7.14 & 38.4 \\
\rowcolor{torange}
\methods (w/ ECT) (Ours) & 1 / 2 & \textbf{3.89} / \textbf{2.75} & 51.2 \\
% iCT~\citep{song2023ict} & 1 & todo & 51.2 \\
% & 2 & todo & 51.2 \\
% ECT~\citep{geng2024ect} & 1 & 5.99 & 51.2 \\
% & 2 & 4.39 & 51.2 \\
% VCT~\citep{silvestri2025vct} & 1 & 5.47 & 51.2 \\
% & 2 & 4.16 & 51.2 \\ 
% \method\ (Ours) & 1 & 7.92 & 38.4 \\
% & 2 & 8.78 & 38.4 \\
% \method+ECT (Ours) & 1 & \textbf{3.89} & 38.4+12.8 \\
% & 2 & \textbf{2.75} & 38.4+12.8 \\
\bottomrule
\end{tabular} %
}

\end{minipage}
\end{comment}
\end{table}


\textbf{ImageNet 512$\times$512}: Table \ref{tab:imagenet-512} compares all
models under Small (S), Medium (M), and Extra-Extra-Large (XXL) sizes. We also provide the training cost in Mimgs for flow map models and \method. 
%
The post-training flow map learning is ECD for our CMT. \method\ significantly outperforms vanilla ECD, again verifying the importance of the mid-training in \method.
%
Overall, our \method\ achieves the second-best 2-step FID in all model scales at a very low cost, 75\% lower than AYF, 87.5\% lower than sCT/ECT, and 93.75\% lower than sCD/ECD.
%
CMT's outstanding cost reduction also holds in terms of training GPU time, as other SOTA methods like sCT, sCD, and AYF all require the model's JVP, whose per-iteration GPU time requirement is higher than CMT's.
%
\method\ is also scalable, when the model grows from S to M to XXL, its FID improves.
%
We use ECD for post-training flow map learning in \methods since it is the only publicly available algorithm at the time of writing. We believe we can further improve \methods results given stronger flow map learning algorithms like sCD and AYF.

\begin{comment}
\begin{table}[t]
\centering
\caption{\small{Sample quality on class-conditional ImageNet 512$\times$512. We report the teacher diffusion models, EDM2 \cite{karras2024edm2} and EDM2 with Auto-Guidance (AutoG) \cite{karras2024edm2autog}. We compare all models under Small (S), Medium (M), and Extra-Extra-Large (XXL) sizes. The cost comparisons for flow map models and \methods are measured under millions of training images (Mimgs).}}
\label{tab:imagenet-512}
\begin{minipage}{0.495\textwidth}
\fontsize{7.6pt}{8.6pt}\selectfont
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip 3pt}c@{\hskip 0pt}c@{\hskip 4pt}c}
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) & \textbf{Cost} ($\downarrow$) \\ % & \textbf{\#Params} \\
\midrule
\multicolumn{3}{l}{\textbf{Teacher Diffusion Models}} \\
\midrule
EDM2-S & 63$\times$2 & 2.23 & N.A. \\
EDM2-M & 63$\times$2 & 2.01 & N.A. \\
% EDM2-L~\citep{karras2024edm2} & 63$\times$2 & 1.88 & N.A. \\
% EDM2-XL~\citep{karras2024edm2} & 63$\times$2 & 1.85 & N.A. \\
% EDM2-XXL~\citep{karras2024edm2} & 63$\times$2 & \textbf{1.81} & 1.5B \\
EDM2-XXL & 63$\times$2 & {1.81} & N.A. \\
EDM2-S~(AutoG) & 63$\times$2 & 1.34 & N.A. \\
EDM2-XXL~(AutoG) & 63$\times$2 & \textbf{1.25} & N.A. \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models}} \\
\midrule 
ECT-S~\citep{geng2024ect} & 1 / 2 & 18.49 / 14.60 & 204.8 \\
ECD-S~\citep{geng2024ect} & 1 / 2 &  14.25 / 6.09 & 409.6\\ 
sCT-S~\citep{lu2025sCM} & 1 / 2 & 10.13 / 9.86 & 204.8 \\
sCD-S~\citep{lu2025sCM} & 1 / 2 & \textbf{3.07} / {2.50} & 409.6 \\
AYF-S~\citep{sabour2025align} & 1 / 2 & \textbf{\textit{3.32}} / \textbf{1.87} & 102.4   \\
\midrule
\multicolumn{3}{l}{\textbf{Consistency Mid-Training (\method)}} \\
\midrule \rowcolor{torange}
\method-S (w/ ECD-S) (Ours) & 1 / 2 &  {{10.38}} / \textbf{\textit{2.48}} & 25.6\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{0.495\textwidth}
\fontsize{6.95pt}{7.95pt}\selectfont
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip 5.5pt}c@{\hskip 0pt}c@{\hskip 4pt}c}
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID}  ($\downarrow$)  & \textbf{Cost}  ($\downarrow$)  \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models}} \\
\midrule 
ECT-M~\citep{geng2024ect} & 1 / 2 & 13.20 / 8.61 & 204.8 \\
ECD-M~\citep{geng2024ect} & 1 / 2 &  12.83 / 5.95 & 409.6\\ 
sCT-M~\citep{lu2025sCM} & 1 / 2 & 5.84 / 5.53 & 204.8 \\
sCD-M~\citep{lu2025sCM} & 1 / 2 & \textbf{2.75} / \textbf{2.26} & 409.6 \\
\midrule
\multicolumn{3}{l}{\textbf{Consistency Mid-Training (\method)}} \\
\midrule \rowcolor{torange}
\method-M (w/ ECD-M) (Ours) & 1 / 2 &  \textbf{\textit{4.11}} / \textbf{\textit{2.39}} & 25.6\\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models}} \\
\midrule 
ECT-XXL~\citep{geng2024ect} & 1 / 2 & 10.82 / 6.56 & 204.8 \\
ECD-XXL~\citep{geng2024ect} & 1 / 2 &  8.47 / 3.38  & 409.6\\ 
sCT-XXL~\citep{lu2025sCM} & 1 / 2 & 4.29 / 3.76  & 204.8\\
sCD-XXL~\citep{lu2025sCM} & 1 / 2 & \textbf{2.28} / \textbf{1.88} & 409.6 \\
% AYF~\citep{sabour2025align} & 1 / 2 & 3.32 / \textbf{1.87}  \\
\midrule
\multicolumn{3}{l}{\textbf{Consistency Mid-Training (\method)}} \\
\midrule \rowcolor{torange}
\method-XXL (w/ ECD-XXL) (Ours) & 1 / 2 &  \textbf{\textit{3.65}} / \textbf{\textit{2.23}} & 25.6 \\
\bottomrule
\end{tabular} %
\end{minipage}
\end{table}
\end{comment}

\begin{table}[t]
\centering
\caption{\small{Sample quality on class-conditional ImageNet 512$\times$512. We report the teacher diffusion models, EDM2 \cite{karras2024edm2} and EDM2 with Auto-Guidance (AutoG) \cite{karras2024edm2autog}. We compare all models under Small (S), Medium (M), and Extra-Extra-Large (XXL) sizes. The cost comparisons for flow map models and \methods are measured under millions of training images (Mimgs).}}
\label{tab:imagenet-512}
\begin{minipage}[t]{0.495\textwidth}
\fontsize{8.0pt}{9.pt}\selectfont
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip 2pt}c@{\hskip 0pt}c@{\hskip 4pt}c}
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID} ($\downarrow$) & \textbf{Cost} ($\downarrow$) \\ % & \textbf{\#Params} \\
\midrule
\multicolumn{3}{l}{\textbf{Teacher Diffusion Models}} \\
\midrule
EDM2-S & 63$\times$2 & 2.23 & N.A. \\
EDM2-M & 63$\times$2 & 2.01 & N.A. \\
% EDM2-L~\citep{karras2024edm2} & 63$\times$2 & 1.88 & N.A. \\
% EDM2-XL~\citep{karras2024edm2} & 63$\times$2 & 1.85 & N.A. \\
% EDM2-XXL~\citep{karras2024edm2} & 63$\times$2 & \textbf{1.81} & 1.5B \\
EDM2-XXL & 63$\times$2 & {1.81} & N.A. \\
EDM2-S~(AutoG) & 63$\times$2 & 1.34 & N.A. \\
EDM2-XXL~(AutoG) & 63$\times$2 & \textbf{1.25} & N.A. \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models - S}} \\
\midrule 
ECT~\citep{geng2024ect} & 1 / 2 & 18.49 / 14.60 & 204.8 \\
ECD~\citep{geng2024ect} & 1 / 2 &  14.25 / 6.09 & 409.6\\ 
sCT~\citep{lu2025sCM} & 1 / 2 & 10.13 / 9.86 & 204.8 \\
sCD~\citep{lu2025sCM} & 1 / 2 & \textbf{3.07} / {2.50} & 409.6 \\
AYF~\citep{sabour2025align} & 1 / 2 & \textbf{\textit{3.32}} / \textbf{1.87} & 102.4   \\
 \rowcolor{torange}
\methods (w/ ECD) (Ours) & 1 / 2 &  {{10.38}} / \textbf{\textit{2.48}} & 25.6\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}[t]{0.495\textwidth}
\fontsize{8.7pt}{9.7pt}\selectfont
% \begin{tabular}{lcc}
\begin{tabular}{l@{\hskip 2pt}c@{\hskip 0pt}c@{\hskip 4pt}c}
\toprule
\textbf{METHOD} & \textbf{NFE} ($\downarrow$) & \textbf{FID}  ($\downarrow$)  & \textbf{Cost}  ($\downarrow$)  \\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models - M}} \\
\midrule 
ECT~\citep{geng2024ect} & 1 / 2 & 13.20 / 8.61 & 204.8 \\
ECD~\citep{geng2024ect} & 1 / 2 &  12.83 / 5.95 & 409.6\\ 
sCT~\citep{lu2025sCM} & 1 / 2 & 5.84 / 5.53 & 204.8 \\
sCD~\citep{lu2025sCM} & 1 / 2 & \textbf{2.75} / \textbf{2.26} & 409.6 \\
 \rowcolor{torange}
\methods (w/ ECD) (Ours) & 1 / 2 &  \textbf{\textit{4.11}} / \textbf{\textit{2.39}} & 25.6\\
\midrule
\multicolumn{3}{l}{\textbf{Flow Map Models - XXL}} \\
\midrule 
ECT~\citep{geng2024ect} & 1 / 2 & 10.82 / 6.56 & 204.8 \\
ECD~\citep{geng2024ect} & 1 / 2 &  8.47 / 3.38  & 409.6\\ 
sCT~\citep{lu2025sCM} & 1 / 2 & 4.29 / 3.76  & 204.8\\
sCD~\citep{lu2025sCM} & 1 / 2 & \textbf{2.28} / \textbf{1.88} & 409.6 \\
% AYF~\citep{sabour2025align} & 1 / 2 & 3.32 / \textbf{1.87}  \\
 \rowcolor{torange}
\methods (w/ ECD) (Ours) & 1 / 2 &  \textbf{\textit{3.65}} / \textbf{\textit{2.23}} & 25.6 \\
\bottomrule
\end{tabular} %
\end{minipage}
\end{table}


\textbf{ImageNet 256$\times$256 and \methods + Mean Flow (MF)}:
We transfer the knowledge in the extra-large pretrained flow matching model SiT-XL/2 (676M) \cite{ma2024sit} to a much smaller Base size model (131M) with a simple \methods step to avoid the cost of training everything from scratch in vanilla MF \cite{geng2025mean}. 
% We also aim to demonstrate that CMT is flexible with teacher and student models that have distinct structures, whereas other methods cannot.

% The training budget is the same as the original MF \cite{geng2025mean}, which is 240 epochs times dataset size (131288080) per epoch. The total is 315 Mimgs.

Given the training budget of 315 Mimgs following MF \cite{geng2025mean}, we compare (1) the baseline of training MF from scratch for 315 Mimgs and (2) \methods mid-training for 1 Mimgs and then use MF for flow map learning for 314 Mimgs.


Quantitatively, MF's 1/2-step FID is 6.37 / 5.35.
In contrast, \method's FID is.
This further proves \method's generality and superior performance.
%
Furthermore, despite the same budget, our \methods GPU training time is shorter than MF since \methods do not require the Jacobian-vector product computation.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/samples_init_compressed.png}
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/samples_init_compressed.png}
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/MF_FINISHED_compressed.png}
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/samples_init_compressed.png}
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/CMT_0_compressed.png}
\includegraphics[width=0.32\linewidth]{ICLR 2026 Template/Figures_MF_Exp/CMT_0_compressed.png}
\caption{Convergence speed comparison between MF \cite{geng2025mean} (upper row) and \methods (Ours, bottom row). 
Left: random initialization. Middle: 1 Mimgs training. Right: Convergence results after 315 Mimgs.}
\label{fig:mf_fid_vs_iter}
\end{figure}
Intuitively, we visualize the intermediate generated image results for both approaches in Figure \ref{fig:mf_fid_vs_iter}.
%
The left column shows the same random initialization for both methods, where the generated images are purely random noise.
%
The middle column shows the generated images of 1 Mimgs training. Vanilla MF still generates pure noise, but \methods converges faster and already learns colorful semantics.
%
Lastly, the right column shows the final converged model's generated images.
%
Thanks to the mid-training's fast convergence, \methods present better FID than vanilla MF.

\subsection{Quantitative Analysis of \methods}
\jc{\textbf{Comparison of Gradient Variances With and Without \method.}}


\textbf{Ablation Study on Bad Teacher}.

\textbf{Ablation Study on Knowledge Distillation (KD) and Slow \method}.
We compare \method's mid-training with KD. KD explicitly focuses on the mapping from noise to the corresponding data only, while \method\ focuses on the entire ODE trajectory consistency. We use the CIFAR10 dataset and train KD with the same settings as \method.
% After the same 38.4 Mimgs training, KD's 1-step FID is 5.62, which is not significantly better than \method's 5.71, while KD's 2-step FID is 100+ since KD neglects the entire ODE trajectory.
% This also demonstrates that \method’s training on the intermediate trajectory does not harm the 1-step FID.
Subsequently, we use ECT to post-train for flow map learning with KD and \method\ initializations for 12.8 Mimgs cost. \method's 1/2 step FID (2.74/1.97) is much better than KD's (3.54/2.19), verifying the benefits of learning intermediate steps.
% Furthermore, on ImageNet 512$\times$512, \method\ achieves a markedly better 2-step FID than its 1-step counterpart, whereas KD is limited to 1-step predictions, constrained by the trade-off between sampling steps and sample quality.
% Hence, for highly challenging high-dimensional datasets, \method’s modeling of the entire ODE trajectory, as opposed to KD’s direct mapping, allows it to serve effectively as a standalone generative model, unlike KD. Notably, \method-M (498M) can outperform ADM \cite{diffusion_beat_gan} of a similar size (559M). Also, \method's 2-step FID outperforms or matches CT's 2-step FID on the S and M size models.


% \textbf{Ablation Study on Gradient Variance}.

% \textbf{Ablation Study on FID versus iteration and Convergence Speed}.

\input{ICLR 2026 Template/cmt_benefits}
